Connectivity constrains quantum codes

Quantum low-density parity-check (LDPC) codes are an important class of quantum error correcting codes. In such codes, each qubit only affects a constant number of syndrome bits, and each syndrome bit only relies on some constant number of qubits. Constructing quantum LDPC codes is challenging. It is an open problem to understand if there exist good quantum LDPC codes, i.e. with constant rate and relative distance. Furthermore, techniques to perform fault-tolerant gates are poorly understood. We present a unified way to address these problems. Our main results are a) a bound on the distance, b) a bound on the code dimension and c) limitations on certain fault-tolerant gates that can be applied to quantum LDPC codes. All three of these bounds are cast as a function of the graph separator of the connectivity graph representation of the quantum code. We find that unless the connectivity graph contains an expander, the code is severely limited. This implies a necessary, but not sufficient, condition to construct good codes. This is the first bound that studies the limitations of quantum LDPC codes that does not rely on locality. As an application, we present novel bounds on quantum LDPC codes associated with local graphs in $D$-dimensional hyperbolic space.

==> applications.tex <==
\emph{Applications}---
At the heart of this section is the definition of a density system, a class of graphs that generalize local graphs in $D$ dimensions.
We borrow from the works of Miller, Thurston, Vavasis and Teng who demonstrated that bounded-density systems have small separators \cite{teng1991phd,miller1991unified,miller1997separators}.

From a practical standpoint, we may wish to design local codes, or at least codes that are as local as possible.
In this section, we address whether a few long-range interactions of high fidelity can significantly improve a local error correcting code.
Unfortunately, the answer appears to be negative and we quantify this statement in the case of $2$-dimensional codes.

Before doing so, we first consider a very general scenario to inform our intuition.
Consider a code family $\scrC$ whose connectivity graphs $\cG = \{G_n\}$ are known to be $s$-separable.
To each graph $G_n \in \cG$ we augment edges $E_{\text{aug}} = E_{\text{aug}}(n)$ which depends on $n$.
We call $\cG'$ the graph family consisting of these augmented graphs.
By removing the endpoints of the edges in $E_{\text{aug}}$, it can be noted that any $G_n' \in \cG'$ is $s'$\mbox{-}separable for $s'(r) = s(r) + 2|E_{\text{aug}}|$.
It follows from Theorem \ref{thm:distancebnd} that $d = O(s'(n)) =  O(s(n) + 2|E_{\text{aug}}|)$. 
As an immediate consequence---if $s(r) = o(r)$, and $\cG$ therefore yields a code family with vanishing relative distance---$\cG'$ cannot yield a good code family unless $|E_{\text{aug}}| = \Omega(n)$.
Any small amount of additional interactions, short- or long-range alike, is always insufficient to significantly improve a code.
This idea of peeling away long-range connections to reveal a poorly connected graph underneath will be a recurring motif in this section.

We now consider ways of making this statement more quantitative and to this end will employ a class of results called geometric separator theorems.
These results explore whether special classes of graphs embedded in $\bbR^D$ have small separators.
We will see how these theorems allow for generalizing the Bravyi-Terhal bound, thereby yielding a stronger notion of locality than bounded-range interactions.


We repeat the definition of the class of neighborhood systems with bounded density $\Delta$, or $\Delta$-density systems for short that describes the notion of interaction range \cite{teng1991phd}.

\begin{figure}[h]
	\centering
	\includegraphics[scale=.3]{pics/density-system}
	\caption{Example of a 2-density system: every green point is contained in at most 2 balls}

\end{figure}

\begin{definition}
    \label{def:densitysystem}
	Let $\scrP = \{p_1,...,p_n\}$ be a set of $n$ points in $\bbR^D$.
	A \emph{$\Delta$-density system} is a set of balls $\Gamma = \{\cB_1,...,\cB_n\}$ such that for all $i \in \{1,...,n\}$,
	\begin{enumerate}
		\item Each $\cB_i$ is centered at $p_i$, and
		\item Each $p_i$ is contained in less than $\Delta$ balls from $\Gamma$.
	\end{enumerate}
    Let $\cC$ be a stabilizer code with a set of generators $\cS = \langle \ssS_i\rangle_{i=1}^{m}$ and $\eta: [n] \to \bbR^D$ be an embedding map on the qubits to the Euclidean space.
    Consider a $\Delta$-density system $\Gamma = \{\cB_i\}_{i=1}^{m} \subset \bbR^{D}$ where we identify $\ssS_i$ with the center of the ball $\cB_i$.
    We say that $(\cC, \eta)$ is associated with a $\Delta$-density system if for every generator $\eta(\supp(\ssS_i)) \subset \cB_i$.
\end{definition}
In other words, we associate a $\Delta$-density system with the stabilizers -- each stabilizer generator $\ssS_i$ is mapped to a ball $\cB_i$.
The constraint on the density limits the extent to which two stabilizers can overlap.
The map $\eta$ ensures that each ball $\cB_i$ contains the support of the stabilizer $\ssS_i$.
We assume that $\eta$ is a uniform embedding, i.e.\ qubits are not clustered in any region.
Equivalently, inside a ball $\cB_i$, there is some constant $\rho$ such that the number of qubits contained within the ball is bounded by $\rho |\cB_i|$.
A density system is not unique; given some system $\Gamma$, any set $\Gamma' = \{\cB'_i\}$ such that $\cB_i \subset \cB'_i$ is also valid.

We repeat the result of \cite{teng1991phd}, Theorem 5.3, page 26 here:
\begin{lemma}
	\label{lem:densitysep}
	Suppose $\Gamma = \{\cB_1,...,\cB_n\}$ is a $\Delta$-density system in $\bbR^D$.
    There is a sphere $S$, such that $S$ intersects at most $c_D \Delta^{1/D}n^{(D-1)/D}$ balls in $\Gamma$ for some constant $c_D > 0$.
    Further $S$ splits $\Gamma$ into sets $\Gamma_{\inside}$ and $\Gamma_{\outside}$ such that the intersection of the balls within the two sets is empty.
\end{lemma}

The core idea of our generalization is that error correcting codes with bounded-range interactions are captured by $\Delta$-density systems.
We now show that Lemma \ref{lem:densitysep} induces a separator for the connectivity graph of $\cC$.

\begin{corollary}
	\label{cor:overlapbound}
	Let $\cC$ be an $\dsl n,k,d \dsr$ code with a connectivity graph whose degree is bounded by some fixed constant $\delta$.
    Suppose we have an embedding $\eta$ such that $(\cC, \eta)$ is associated with a $\Delta$-density system.
    Then we have $d = O(\Delta^{1/D}n^{(D-1)/D)})$.
\end{corollary}

\begin{proof}
    As we are working with a $\Delta$-density system, Lemma \ref{lem:densitysep} guarantees a separator $S$ of size $O(n^{1-1/D})$.
	The separator $S$ splits the set of balls $\Gamma = \{\cB_i\}$ into $\Gamma_{\inside} \sqcup \Gamma_{\text{sep}} \sqcup \Gamma_{\outside}$ such that balls in $\Gamma_{\inside}$ do not overlap balls in $\Gamma_{\outside}$.

    Therefore, no qubit belongs simultaneously to a generator associated with a ball in $\Gamma_{\inside}$, and a generator associated with a ball in $\Gamma_{\outside}$.
    We naturally conclude that $S$ induces a separator in the connectivity graph.
    Consider $S'$ the set of qubits connected to generators associated with balls that overlap with $S$. 
	
	Since the connectivity graph has bounded degree with maximum degree $\delta$, it follows that $|S'| \leq \delta |S|$.
    Therefore we can now use Theorem \ref{thm:distancebnd} to obtain the desired result.
\end{proof}

We note that the Bravyi-Terhal bound follows by observing that a local code in $D$ dimensions is a constant-density system.
Going further, Corollary \ref{cor:overlapbound} allows us to quantify the non-locality of a generator in $D$ dimensions.
A generator $\ssS_i$ that is contained in many balls $\cB_j$ for $j \neq i$ increases $\Delta$ which is a necessary condition for a large distance.
However, we would not expect a single non-local generator to significantly improve the separability of the connectivity graph.

One proposal to implement a code with nonlocal connectivity is to use a \emph{stacked} layout.
In such a layout, the stabilizers are assigned to different layers in a stack based on the radius within which they are supported.
We wish to implement a majority of the checks using only local interactions and these form the bottom most layer of the stack.
The remaining checks have varying degrees of nonlocality, but the number of such checks decreases as we move further up the stack.

Suppose we wished to design an error correcting code using a stacked layout in $2$-dimensions.
Consider the following proposal where qubits are laid out on a square grid of size $n = 2^{l_m} \times 2^{l_m}$ as shown in fig.~\ref{fig:stacked-pre}.
In total, there are $l_m$ layers in this stack, where the generators at level $l$ act within a ball of radius $r_l = 2^{l}/\sqrt{2}$.
At the very top, we have a highly nonlocal stabilizer associated with a ball of radius $r_{l_m} = 2^{l_m}/\sqrt{2}$.
To be clear, while the stabilizer in the top-most layer has a radius of $r_{l_m}$, it still only jointly checks some constant number of qubits.
The radius merely constrains where these qubits are allowed to be located.
In the next layer we have $4$ stabilizers but these stabilizers are each only supported within a ball of radius $r_{l-1} = 2^{l-1}/\sqrt{2}$.
This proceeds until we hit the very last layer---there are $4^{l_m-l}$ such generators in layer $l$---until we hit layer $0$ which consists of stabilizers supported entirely within a ball of constant radius.
It follows that the majority of the stabilizers are in the last layer or in other words, the majority of stabilizers are local with $r = O(1)$ locality.
Indeed, layer $0$ contains at least $3$ times as many stabilizers as the total number of stabilizers in all other $l_m-1$ layers combined.

\begin{theorem}
    \label{lem:stack-lim}
    Let $\cC$ be an $\dsl n,k,d \dsr$ code whose qubit and check degrees are bounded by $\delta_Q$ and $\delta_C$ respectively.
    Suppose $\cC$ can be implemented by a $2$-dimensional stack architecture as described above.
    Then the distance of the code obeys $d = O(n^{2/3})$.
\end{theorem}
\begin{proof}
    We will prove that if $\cC$ can be implemented by a stack, then it is a bounded-density system.
    The embedding map $\eta$ is implicit in this case as the qubits are located on the vertices of the integer grid.
    It follows that the qubits are not concentrated in any one region of space.
    Each layer $0 \leq l \leq l_m$ defines at most $4^{l_m - l}$ stabilizers with a radius of $r_l = 2^{l}/\sqrt{2}$.
    Together, these form the balls $\cB_i$ of the density system and the centers are the points $p_i$ identified with stabilizer generators $\ssS_i$.

    The proof proceeds in two stages.

    \textbf{Step 1:}
    We shall remove the support of stabilizers that contribute to a high density.
    These are clearly the stabilizers in the upper layers as they have the farthest reach.
    Consider the stabilizers in the layers $\frac{1}{3}l_m  \leq l \leq l_m$.
    By removing all the qubits connected to these stabilizers, we remove $O(n^{2/3})$ fraction of qubits.
    This is because the number of qubits we remove is upper bounded by
    \begin{equation}
        \delta_C \sum_{l=\frac{1}{3}l_m}^{l_m} 4^{l_m-l} = O(n^\frac{2}{3})~.
    \end{equation}

    \textbf{Step 2:}
    We now focus on the remaining code and our intent is to bound its density.
    Let each stabilizer generator $\ssS_i$ correspond to a point $p_i$ in the grid.
    We are interested in upper-bounding the number of balls $\cB_j$, $j\neq i$, such that $p_i \in \cB_j$.
    Let $\cT_{p_i}(l) = \{\ssS_j\}_j \subseteq \cS$ be the subset of generators in the $l$-th level such that the corresponding balls $\cB_j$, $j \neq i$, contain $p_i$.
    We shall first upper bound $\mathopen|\cT_{p_i}(l)\mathclose|$.
    
    The number of qubits contained within these balls is at most $\rho \mathopen|\union_j \cB_j\mathclose|$, where $\rho$ is some constant factor which measures the density of qubits in $2$ dimensions.
    The number of stabilizer generators these qubits are connected to is at most $\delta_Q \rho \mathopen|\union_j \cB_j\mathclose|$.
    The number of stabilizer generators in $\cT_{p_i}(l)$ is simply $\mathopen|\cT_{p_i}(l)\mathclose|$.
    This implies that we have $\delta_Q \rho \mathopen|\union_j \cB_j\mathclose| \geq |\cT_{p_i}(l)|$.
    We achieve equality if and only if all the qubits in the balls are connected exclusively to these stabilizer generators $\cT_{p_i}(l)$ in level $l$.

    Since the radius of each ball $\cB_j$ is at most $r_l$, the union of all the balls $\union_i \cB_j$ is contained within a ball of radius $2r_l$.
    Therefore, $\mathopen|\union_j \cB_j\mathclose| \leq 4 \pi r_l^2$.
    We can put these ingredients together to bound the density as
    \begin{align}
        |\cT_{p_i}(l)| = O(r_l^2) = O(4^{l})~.
    \end{align}

    We can therefore compute an upper-bound on the density $\Delta$ by summing the density contribution of every level
    \begin{align}
        \Delta \leq 2 \pi \sum_{l=0}^{l=l_m/3}|\cT_p(l)| = \sum_{l=0}^{l=l_m/3} O(4^l) = O(n^{1/3})~.
    \end{align}
    This shows that the remaining code has bounded density.
    From Lemma \ref{lem:densitysep}, it has a separator of size at most $O(\Delta^{1/2}n^{1/2}) = O(n^{2/3})$.

    The size of the separator for the entire density system corresponding to the code is then the total of the contributions of the first and second portions which is simply $O(n^{2/3})$.
    
    From Corollary \ref{cor:overlapbound}, we obtain the desired bound on the distance $d = O(n^{2/3})$.
\end{proof}
